ShapeMOD: Macro Operation Discovery for 3D Shape Programs

A popular way to create detailed yet easily controllable 3D shapes is via procedural modeling, i.e. generating geometry using programs. Such programs consist of a series of instructions along with their associated parameter values. To fully realize the benefits of this representation, a shape program should be compact and only expose degrees of freedom that allow for meaningful manipulation of output geometry. One way to achieve this goal is to design higher-level macro operators that, when executed, expand into a series of commands from the base shape modeling language. However, manually authoring such macros, much like shape programs themselves, is difficult and largely restricted to domain experts. In this paper, we present ShapeMOD, an algorithm for automatically discovering macros that are useful across large datasets of 3D shape programs. ShapeMOD operates on shape programs expressed in an imperative, statement-based language. It is designed to discover macros that make programs more compact by minimizing the number of function calls and free parameters required to represent an input shape collection. We run ShapeMOD on multiple collections of programs expressed in a domain-specific language for 3D shape structures. We show that it automatically discovers a concise set of macros that abstract out common structural and parametric patterns that generalize over large shape collections. We also demonstrate that the macros found by ShapeMOD improve performance on downstream tasks including shape generative modeling and inferring programs from point clouds. Finally, we conduct a user study that indicates that ShapeMOD's discovered macros make interactive shape editing more efficient.

==> 05-results.tex <==
\section{Results and Evaluation}
\label{sec:results}

We run experiments on categories of manufactured shapes from CAD models in PartNet, and use the same data parsing procedure as described in ShapeAssembly on the categories of Chairs, Tables and Storage.

We run this operation discovery procedure on two 'base' versions of ShapeAssembly. The default one contains just the cuboid and attach operators. The RTS version contains the previously manually defined macro functions of reflect, translate and squeeze. In all experiments, we compare our Operation Discovery procedure to the base language it started from. 

\subsection{Discovered Operators}

\begin{table}[t!]
    \centering    
    \setlength{\tabcolsep}{2pt}
    \small
    \begin{tabular}{@{}llccccc@{}}
        \toprule
        \textbf{Category} & \textbf{Method} & \textbf{\# Funcs} & \textbf{\# Lines} & \textbf{\# Disc Params} & \textbf{\# Cont Params}  \\
        \midrule
        \multirow{4}{*}{\emph{Chair}}
        & Base &  \\
        & OpDisc &    \\
        & Base(RTS) &   \\
        & OpDisc(RTS) &   \\
        \midrule
        \multirow{4}{*}{\emph{Table}}
        & Base &   \\
        & OpDisc &    \\
        & Base(RTS) &   \\
        & OpDisc(RTS) &    \\
        \midrule
        \multirow{4}{*}{\emph{Storage}}
        & Base &  \\
        & OpDisc &    \\
        & Base(RTS) &   \\
        & OpDisc(RTS) &  \\
        \bottomrule
    \end{tabular}
    \caption{Measuring how well different language can represent a dataset of shape programs. All metrics except number of functions are averaged across each data instance. For \# lines and parameters, lower numbers are better. }
    \label{tab:prog_stats}
\end{table}

We compare how well the discovered languages from our procedure can represent a dataset of 3D Shape programs in Table \ref{tab:prog_stats}. With the newly discovered languages, we can represent data instances across the data set much more compactly just by adding a small number of parameterized functions. Introduce some, small, parametric error, but no structural errors. \\

\begin{figure}
  \includegraphics[width=\linewidth]{figs/placeholder.pdf}
\caption{Some examples of discovered functions, the structures they create, their internal logic, their assigned names, and what happens when their parameters are modified.}
\label{fig:qual_funcs}
\end{figure}

In Figure \ref{fig:qual_funcs} we show some of the discovered abstractions. \\ \\


\begin{table}[t!]
    \centering    
    \setlength{\tabcolsep}{2pt}
    \small
    \begin{tabular}{@{}cccc@{}}
        \toprule
        & & \textbf{Mode \%} & \textbf{Singleton \%} \\
        \midrule
        & Manual Funcs &  \\
        & Discovered Funcs &    \\
        & Manual Params &   \\
        & Discovered Params & \\
    \bottomrule
    \end{tabular}
    \caption{ We compare how semantically consistent discovered macro functions and their parameter slots are to manually designed macro functions taken from ShapeAssembly. Mode \% is the frequency of the most common response. Singleton \% is the freuqency of singleton responses.}
    \label{tab:abs_comp}
\end{table}

We run an experiment where we show a group of users examples of our discovered abstractions in use, and then ask them to give names to the abstraction and its parameter slots. We compare discovered abstractions to the manually designed abstractions from ShapeAssembly (as an upper bound), and report the consistency of this naming information in Table \ref{tab:abs_comp}. As there is reasonable consistency, this is evidence that the abstractions we find are semantically interpretable. 

\subsection{Generating 3D Shapes}

We train a generative model on the same set of programs expressed in different languages across the different partnet categories of interest. 

\subsubsection{Analysis of Quality}

\begin{figure}
  \includegraphics[width=\linewidth]{figs/placeholder.pdf}
\caption{Unconditional Generations of Shapes + Programs with and without the operation discovery procedure.}
\label{fig:qual_examples}
\end{figure}

We share some qualitative examples of shape and program unconditional generations of generative models trained with and without the discovered operators in figure \ref{fig:qual_examples}.

\begin{table}[t!]
    \centering    
    \setlength{\tabcolsep}{2pt}
    \small
    \begin{tabular}{@{}cccc@{}}
      
      \textbf{Method} & \textbf{Validity} & \textbf{Editability} & \textbf{Structural Complexity}  \\
      \midrule
        Base(RTS) &   \\ 
        OpDisc(RTS) &   \\
       \bottomrule
    \end{tabular}
    \caption{User study comparing generative model train with base (RTS) language versus discovered language from operation discovery procedure. For each metric, the average score of uncoditional generations on a 1-5 scale is reported.}
    \label{tab:us_quality}
\end{table}

We run a user study asking individuals to compare generations (i.e. shapes and programs) from the two methods on shape validity, perceived editability, and structural complexity, results are reported in Table \ref{tab:us_quality}.


\begin{table}[t!]
    \centering    
    \setlength{\tabcolsep}{2pt}
    \small
    \begin{tabular}{@{}llcccc@{}}
        \toprule
        \textbf{Category} & \textbf{Method} & \textbf{\% rooted}$\;\Uparrow$ & \textbf{\% stable}$\;\Uparrow$ & \textbf{\% fool}$\;\Uparrow$ & \textbf{FD}$\;\Downarrow$ \\
        \midrule
        \multirow{4}{*}{\emph{Chair}}
        & Base &  \\
        & OpDisc &    \\
        & Base(RTS) &   \\
        & OpDisc(RTS) &   \\
        \midrule
        \multirow{4}{*}{\emph{Table}}
        & Base &   \\
        & OpDisc &    \\
        & Base(RTS) &   \\
        & OpDisc(RTS) &    \\
        \midrule
        \multirow{4}{*}{\emph{Storage}}
        & Base &  \\
        & OpDisc &    \\
        & Base(RTS) &   \\
        & OpDisc(RTS) &  \\
        \bottomrule
    \end{tabular}
    \caption{Comparing the quality of generated samples.}
    \label{tab:prog_stats}
\end{table}

Quantitatively we compare the quality of the generative model with the same metrics as in ShapeAssembly in Table \ref{tab:prog_stats}.

\subsubsection{Analysis of Variability}

\begin{table}[t!]
    \centering    
    % \small
    \footnotesize
    \setlength{\tabcolsep}{1pt}
    %\vspace{-1em}
    \begin{tabular}{@{}llcccccc@{}}
        \toprule
        & & \multicolumn{2}{c}{\emph{Generalization}} & \multicolumn{2}{c}{\emph{Coverage}} & \multicolumn{2}{c}{\emph{Variety}}
        \\
        & & \multicolumn{2}{c}{NND to Train$\;\Uparrow$} & \multicolumn{2}{c}{NND from Val$\;\Downarrow$} & \multicolumn{2}{c}{NND to Self$\;\Uparrow$}
        \\
        \textbf{Category} & \textbf{Method} & 
        \textbf{CD} & \textbf{ED} &
        \textbf{CD} & \textbf{ED} &
        \textbf{CD} &\textbf{ED}
        \\
        \midrule
        \multirow{4}{*}{\emph{Chair}}
        & Base &  \\
        & OpDisc &    \\
        & Base(RTS) &   \\
        & OpDisc(RTS) &  \\
        \midrule
        \multirow{4}{*}{\emph{Table}}
        & Base &  \\
        & OpDisc &    \\
        & Base(RTS) &   \\
        & OpDisc(RTS) &  \\
        \midrule
        \multirow{4}{*}{\emph{Storage}}
        & Base &  \\
        & OpDisc &    \\
        & Base(RTS) &   \\
        & OpDisc(RTS) &  \\
        \bottomrule
    \end{tabular}
    \caption{Using Chamfer Distance (CD) and Program Edit Distance (ED), we check how well generative models generalize from the training set, cover the validation set, and have variability within their own set.}
    \label{tab:variability}
\end{table}

To check how macros impact the variability of a generative model we look at the same metrics as in ShapeAssembly -- on both geometric and structural distance metrics in Table \ref{tab:variability}. 


\subsection{3D Shape Editing}

Experiment where we take a ground-truth shape, find a parametric variation (achievable in both lower-level and high-level abstractions), then give it to the user as a goal direction editing task (by manipulating levers).

\begin{table}[t!]
    \centering    
    \setlength{\tabcolsep}{2pt}
    \footnotesize
    \begin{tabular}{@{}ccccccc@{}}
      
      \textbf{Method} & \textbf{Completion \%} & \textbf{Geom Dist} & \textbf{Time} & \textbf{\# Edits} & \textbf{Satisfied} & \textbf{Difficulty} \\
      \midrule
        Base & \\
        OpDisc & \\
        Base(RTS) & \\ 
        OpDisc(RTS) & \\
       \bottomrule
    \end{tabular}
    \caption{Results of user study on goal directed editing tasks trying to make shape A into shape B through parametric variation. Completion \% is the percentage of the time the edit was succesful (within certain geometric distance). Geom dist is the average geometric distance from final edit to target. Time is the amount of time taken on succesfull runs. \# of edits records the number of times a parameter was adjusted, for a given edit sequence. Satisfied and Difficulty are on a 1-5 scale, entered by user after each edit sequence.}
    \label{tab:us_edit}
\end{table}
 
\begin{figure}
  \includegraphics[width=\linewidth]{figs/placeholder.pdf}
\caption{Results of goal directed edit sequences with and without macro functions.}
\label{fig:qual_edits}
\end{figure}

We show quantiative results from this experiment in Table \ref{tab:us_edit} and qualitative results of edits found in Figure \ref{fig:qual_edits}. 



